The Carnegie-Irvine Galaxy Survey. VII. Constraints on the Origin of S0 Galaxies from Their Photometric Structure

Using high-quality optical images from the Carnegie-Irvine Galaxy Survey, we perform multi-component decompositions of S0 galaxies to derive accurate structural parameters to constrain their physical origin. Many S0s do not host prominent bulges. S0 galaxies have a broad distribution of bulge-to-total ratios ($B/T$) and S\'ersic indices ($n$), with average values of $B/T=0.34\pm0.15$ and $n=2.62\pm1.02$, qualitatively consistent with the notion that S0s define a parallel sequence with and may have evolved from spiral galaxies. This is further reinforced by the incidence of bars and lenses in S0s, which when compared with the statistics in spirals, supports the idea that lenses are demised bars. However, despite their wide range of prominence, the bulges of S0s form a surprisingly uniform sequence on both the Kormendy and fundamental plane relations. There is no evidence for population dichotomy or other indications of differentiation into classical and pseudo bulges. Most of the S0s reside in the field and in groups; cluster environment is not a necessary condition for S0 production. The properties of S0 bulges show little correlation with environmental indicators, after the dependence of galaxy stellar mass on environment is taken into account. As the bulges of late-type spirals and S0s are intrinsically different, and environmental effects that may account for such evolution appear to be minimal, we conclude that late-type spirals are not plausible progenitors of S0s. The bulges of S0s likely formed at an early epoch, after which secular processes contributed little to their subsequent evolution.

==> figset1.tex <==

\figsetstart
\figsetnum{1}
\figsettitle{Best-fit models of CGS S0s}

\figsetgrpstart
\figsetgrpnum{1.1}
\figsetgrptitle{ESO 221-G026}
\figsetplot{figset_s0/ESO221-G026}
\figsetgrpnote{Best-fit model of ESO 221-G026. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.2}
\figsetgrptitle{ESO 442-G026}
\figsetplot{figset_s0/ESO442-G026}
\figsetgrpnote{Best-fit model of ESO 442-G026. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.3}
\figsetgrptitle{ESO 507-G025}
\figsetplot{figset_s0/ESO507-G025}
\figsetgrpnote{Best-fit model of ESO 507-G025. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.4}
\figsetgrptitle{IC 2006}
\figsetplot{figset_s0/IC2006}
\figsetgrpnote{Best-fit model of IC 2006. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.5}
\figsetgrptitle{IC 2035}
\figsetplot{figset_s0/IC2035}
\figsetgrpnote{Best-fit model of IC 2035. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.6}
\figsetgrptitle{IC 4329}
\figsetplot{figset_s0/IC4329}
\figsetgrpnote{Best-fit model of IC 4329. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.7}
\figsetgrptitle{IC 4991}
\figsetplot{figset_s0/IC4991}
\figsetgrpnote{Best-fit model of IC 4991. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.8}
\figsetgrptitle{IC 5267}
\figsetplot{figset_s0/IC5267}
\figsetgrpnote{Best-fit model of IC 5267. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.9}
\figsetgrptitle{NGC 254}
\figsetplot{figset_s0/NGC0254}
\figsetgrpnote{Best-fit model of NGC 254. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.10}
\figsetgrptitle{NGC 584}
\figsetplot{figset_s0/NGC0584}
\figsetgrpnote{Best-fit model of NGC 584. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.11}
\figsetgrptitle{NGC 936}
\figsetplot{figset_s0/NGC0936}
\figsetgrpnote{Best-fit model of NGC 936. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.12}
\figsetgrptitle{NGC 1201}
\figsetplot{figset_s0/NGC1201}
\figsetgrpnote{Best-fit model of NGC 1201. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.13}
\figsetgrptitle{NGC 1302}
\figsetplot{figset_s0/NGC1302}
\figsetgrpnote{Best-fit model of NGC 1302. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.14}
\figsetgrptitle{NGC 1326}
\figsetplot{figset_s0/NGC1326}
\figsetgrpnote{Best-fit model of NGC 1326. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.15}
\figsetgrptitle{NGC 1380}
\figsetplot{figset_s0/NGC1380}
\figsetgrpnote{Best-fit model of NGC 1380. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.16}
\figsetgrptitle{NGC 1386}
\figsetplot{figset_s0/NGC1386}
\figsetgrpnote{Best-fit model of NGC 1386. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.17}
\figsetgrptitle{NGC 1387}
\figsetplot{figset_s0/NGC1387}
\figsetgrpnote{Best-fit model of NGC 1387. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.18}
\figsetgrptitle{NGC 1400}
\figsetplot{figset_s0/NGC1400}
\figsetgrpnote{Best-fit model of NGC 1400. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.19}
\figsetgrptitle{NGC 1411}
\figsetplot{figset_s0/NGC1411}
\figsetgrpnote{Best-fit model of NGC 1411. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.20}
\figsetgrptitle{NGC 1527}
\figsetplot{figset_s0/NGC1527}
\figsetgrpnote{Best-fit model of NGC 1527. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.21}
\figsetgrptitle{NGC 1533}
\figsetplot{figset_s0/NGC1533}
\figsetgrpnote{Best-fit model of NGC 1533. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.22}
\figsetgrptitle{NGC 1537}
\figsetplot{figset_s0/NGC1537}
\figsetgrpnote{Best-fit model of NGC 1537. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.23}
\figsetgrptitle{NGC 1543}
\figsetplot{figset_s0/NGC1543}
\figsetgrpnote{Best-fit model of NGC 1543. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.24}
\figsetgrptitle{NGC 1553}
\figsetplot{figset_s0/NGC1553}
\figsetgrpnote{Best-fit model of NGC 1553. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.25}
\figsetgrptitle{NGC 1574}
\figsetplot{figset_s0/NGC1574}
\figsetgrpnote{Best-fit model of NGC 1574. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.26}
\figsetgrptitle{NGC 1726}
\figsetplot{figset_s0/NGC1726}
\figsetgrpnote{Best-fit model of NGC 1726. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.27}
\figsetgrptitle{NGC 1947}
\figsetplot{figset_s0/NGC1947}
\figsetgrpnote{Best-fit model of NGC 1947. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.28}
\figsetgrptitle{NGC 2217}
\figsetplot{figset_s0/NGC2217}
\figsetgrpnote{Best-fit model of NGC 2217. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.29}
\figsetgrptitle{NGC 2640}
\figsetplot{figset_s0/NGC2640}
\figsetgrpnote{Best-fit model of NGC 2640. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.30}
\figsetgrptitle{NGC 2695}
\figsetplot{figset_s0/NGC2695}
\figsetgrpnote{Best-fit model of NGC 2695. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.31}
\figsetgrptitle{NGC 2698}
\figsetplot{figset_s0/NGC2698}
\figsetgrpnote{Best-fit model of NGC 2698. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.32}
\figsetgrptitle{NGC 2781}
\figsetplot{figset_s0/NGC2781}
\figsetgrpnote{Best-fit model of NGC 2781. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.33}
\figsetgrptitle{NGC 2784}
\figsetplot{figset_s0/NGC2784}
\figsetgrpnote{Best-fit model of NGC 2784. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.34}
\figsetgrptitle{NGC 2983}
\figsetplot{figset_s0/NGC2983}
\figsetgrpnote{Best-fit model of NGC 2983. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.35}
\figsetgrptitle{NGC 3056}
\figsetplot{figset_s0/NGC3056}
\figsetgrpnote{Best-fit model of NGC 3056. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.36}
\figsetgrptitle{NGC 3100}
\figsetplot{figset_s0/NGC3100}
\figsetgrpnote{Best-fit model of NGC 3100. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.37}
\figsetgrptitle{NGC 3108}
\figsetplot{figset_s0/NGC3108}
\figsetgrpnote{Best-fit model of NGC 3108. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.38}
\figsetgrptitle{NGC 3271}
\figsetplot{figset_s0/NGC3271}
\figsetgrpnote{Best-fit model of NGC 3271. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.39}
\figsetgrptitle{NGC 3892}
\figsetplot{figset_s0/NGC3892}
\figsetgrpnote{Best-fit model of NGC 3892. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.40}
\figsetgrptitle{NGC 3904}
\figsetplot{figset_s0/NGC3904}
\figsetgrpnote{Best-fit model of NGC 3904. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.41}
\figsetgrptitle{NGC 4024}
\figsetplot{figset_s0/NGC4024}
\figsetgrpnote{Best-fit model of NGC 4024. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.42}
\figsetgrptitle{NGC 4033}
\figsetplot{figset_s0/NGC4033}
\figsetgrpnote{Best-fit model of NGC 4033. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.43}
\figsetgrptitle{NGC 4373A}
\figsetplot{figset_s0/NGC4373A}
\figsetgrpnote{Best-fit model of NGC 4373A. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.44}
\figsetgrptitle{NGC 4546}
\figsetplot{figset_s0/NGC4546}
\figsetgrpnote{Best-fit model of NGC 4546. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.45}
\figsetgrptitle{NGC 4684}
\figsetplot{figset_s0/NGC4684}
\figsetgrpnote{Best-fit model of NGC 4684. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.46}
\figsetgrptitle{NGC 4697}
\figsetplot{figset_s0/NGC4697}
\figsetgrpnote{Best-fit model of NGC 4697. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.47}
\figsetgrptitle{NGC 4802}
\figsetplot{figset_s0/NGC4802}
\figsetgrpnote{Best-fit model of NGC 4802. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.48}
\figsetgrptitle{NGC 4825}
\figsetplot{figset_s0/NGC4825}
\figsetgrpnote{Best-fit model of NGC 4825. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.49}
\figsetgrptitle{NGC 4856}
\figsetplot{figset_s0/NGC4856}
\figsetgrpnote{Best-fit model of NGC 4856. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.50}
\figsetgrptitle{NGC 4984}
\figsetplot{figset_s0/NGC4984}
\figsetgrpnote{Best-fit model of NGC 4984. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.51}
\figsetgrptitle{NGC 5026}
\figsetplot{figset_s0/NGC5026}
\figsetgrpnote{Best-fit model of NGC 5026. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.52}
\figsetgrptitle{NGC 5266}
\figsetplot{figset_s0/NGC5266}
\figsetgrpnote{Best-fit model of NGC 5266. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.53}
\figsetgrptitle{NGC 5333}
\figsetplot{figset_s0/NGC5333}
\figsetgrpnote{Best-fit model of NGC 5333. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.54}
\figsetgrptitle{NGC 6673}
\figsetplot{figset_s0/NGC6673}
\figsetgrpnote{Best-fit model of NGC 6673. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.55}
\figsetgrptitle{NGC 6684}
\figsetplot{figset_s0/NGC6684}
\figsetgrpnote{Best-fit model of NGC 6684. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.56}
\figsetgrptitle{NGC 6893}
\figsetplot{figset_s0/NGC6893}
\figsetgrpnote{Best-fit model of NGC 6893. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.57}
\figsetgrptitle{NGC 6942}
\figsetplot{figset_s0/NGC6942}
\figsetgrpnote{Best-fit model of NGC 6942. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.58}
\figsetgrptitle{NGC 7049}
\figsetplot{figset_s0/NGC7049}
\figsetgrpnote{Best-fit model of NGC 7049. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.59}
\figsetgrptitle{NGC 7079}
\figsetplot{figset_s0/NGC7079}
\figsetgrpnote{Best-fit model of NGC 7079. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.60}
\figsetgrptitle{NGC 7144}
\figsetplot{figset_s0/NGC7144}
\figsetgrpnote{Best-fit model of NGC 7144. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.61}
\figsetgrptitle{NGC 7192}
\figsetplot{figset_s0/NGC7192}
\figsetgrpnote{Best-fit model of NGC 7192. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.62}
\figsetgrptitle{NGC 7377}
\figsetplot{figset_s0/NGC7377}
\figsetgrpnote{Best-fit model of NGC 7377. Same conventions as in Figure~\ref{fig:exam}.}
\figsetgrpend

\figsetend
\begin{figure*}[h]
  \epsscale{1.15}
  \plotone{figset_s0/NGC0936}
  \caption{Best-fit model of NGC~936. The left panels display the isophotal analysis of the 2D image
    fitting. From top to bottom, the panels show radial profiles of the 4th harmonic deviations from
    ellipse ($A_{4}$ and $B_{4}$), the ellipticity ($\epsilon$), the position angle (PA), the
    $R$-band surface brightness ($\mu_{R}$), and the fitting residuals ($\bigtriangleup\mu_{R}$).
    Profiles of the data image, the model image, and the individual components are encoded
    consistently with different symbols, line styles, and colors, which are explained in the
    legends. The text on the right side of the legends gives detailed information of each component;
    from left to right, each column describes the radial profile functions (PSF, \sersic{},
    exponential, and modified Ferrer) and whether they are complete or truncated (blank for
    complete, ``\textbackslash@$r_{\mathrm{break}} +\bigtriangleup r_{\mathrm{soft}}$'' for outer
    truncation, and ``/@$r_{\mathrm{break}}-\bigtriangleup r_{\mathrm{soft}}$'' for inner
    truncation), the light fractions, the characteristic surface brightness (effective surface
    brightness $\mu_{e}$ for the bulge and central surface brightness $\mu_{0}$ for the others), the
    shape parameters of the radial profiles (\sersic{} index $n$ for the \sersic{} function and
    $\alpha\,\&\,\beta$ for the modified Ferrer function), the characteristic radii (effective
    radius $r_{e}$ for the \sersic{} function, outer boundary $r_{\mathrm{out}}$ for the modified
    Ferrer function, and scale length $r_{s}$ for the exponential function), the axis ratios ($q$),
    and the position angles (PA). The parameters can be constrained to be the same (braces) and/or
    fixed (brackets). Note that the surface brightness profile of the model is generated by fixing
    the geometric parameters to those of the data surface brightness profile, and the surface
    brightness profiles of individual components are generated along their major axes; hence, the
    model surface brightness profile is not a simple summation of those of the individual
    components. The right panels display, from top to bottom, the grayscale $R$-band data image, the
    best-fit model image, and the residual image. The images are shown using the same logarithmic
    stretch for the data and model image, and histogram equalization stretch for the residual
    image. All images are cropped to have the same size of $1.5D_{25}$ and are centered on the
    galaxy centroid, with north up and east to the left. \\(The complete figure set of 62 images is
    available in the online journal.) \label{fig:exam}}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: paper2_sub
%%% End:

%  LocalWords:  grayscale ellipticity expdisk Ferrer isophotal PAs

